Multiversion Hindsight Logging for Continuous Training

Production Machine Learning involves continuous training: hosting multiple versions of models over time, often with many model versions running at once. When model performance does not meet expectations, Machine Learning Engineers (MLEs) debug issues by exploring and analyzing numerous prior versions of code and training data to identify root causes and mitigate problems. Traditional debugging and logging tools often fall short in managing this experimental, multi-version context. FlorDB introduces Multiversion Hindsight Logging, which allows engineers to use the most recent version's logging statements to query past versions, even when older versions logged different data. Log statement propagation enables consistent injection of logging statements into past code versions, regardless of changes to the codebase. Once log statements are propagated across code versions, the remaining challenge in Multiversion Hindsight Logging is to efficiently replay the new log statements based on checkpoints from previous runs. Finally, a coherent user experience is required to help MLEs debug across all versions of code and data. To this end, FlorDB presents a unified relational model for efficient handling of historical queries, offering a comprehensive view of the log history to simplify the exploration of past code iterations. We present a performance evaluation on diverse benchmarks confirming its scalability and the ability to deliver real-time query responses, leveraging query-based filtering and checkpoint-based parallelism for efficient replay.

==> sections/authoring_ui.tex <==
\section{Tractable Query Patterns}\label{sec:q_authoring}

Do you want to condition the loss being above some threshold?
Prompt. Want to click on red column? Before you click, have you introduced any filters
COST advisor and cost minimization wizard, not AI just a set of questions;
query authoring.

Spreadsheet markup of the result,
Here's what you can do, Add a UI figure.
If we imagine the UI, we can imagine what to talk about.

Counter-intuitive: by hindsight-logging more stuff,
I have more conditions to filter on,
and I can speed up my query.
Encourage developer to add extra
hindsight logging statements
before query.

Add WHERE clauses on cheap columns.
So we can avoid expensive columns.
Best practices for querying,
one can imagine UI ...
Crisp about patterns and anti-patterns.
Patterns for tractable queries. How do you stay above water? "one could imagine tools…"


==> sections/pred_pushdown.tex <==
\subsection{Physical Query Operators}\label{sec:query_exec}
\begin{figure}
      \centering
      \includegraphics[width=0.5\textwidth]{images/quad/error.png}
      \caption{Physical Query Operators and Associated Errors}
      \label{fig:costEstimate}
\end{figure}


\jmh{Add discussion about background server process here.}
\jmh{More detail needed here. What are the arguments we can pass into each operator? How do they limit the scope of replay? I'd assume we can only calibrate correctly because the arguments we pass in are directly related to the execution ... you should clarify that point. By contrast, in a traditional index we don't know how many I/Os will be needed to satisfy a range query (or a point query on duplicated data). Why doesn't that problem come up here?}
\begin{itemize}
      \item $DP$: Index Scan: As the default replay operator, $DP$ executes the entire model training code, traversing the main epoch loop but bypassing the nested training loop by loading checkpoints. This operator is particularly useful when hindsight logging statements are incorporated into the model validation section of the code.
      \item $DP^*$ Index Lookup: \jmh{lookup on what?} When parameterized for model evaluation, this replay operator also executes the complete model training code but skips the main loop by loading the final checkpoint from training. Flor resorts to this operator when hindsight logging statements are added into the model evaluation or testing section of the code, which typically follows the main loop.
      \item $DP_{i,n}$: Range Scan: This operator can be parameterized by the number of workers (n), and work partition (i). \jmh{what is a work partition?} It holds value for parallelizing model training replay, as well as for selective replay. For instance, if the model developer wishes to observe the tensor histograms at a specific iteration, FlorDB can adjust the number of workers to match the number of epochs, and step into the desired iteration. Flor employs this replay operator for the most granular logging: whenever model developers introduce hindsight logging statements into the nested training loop.

\end{itemize}

\jmh{Perhaps note that replay can easily be the bottleneck in FlorDB query processing, 
as opposed to traditional concerns of minimizing the cost of ``downstream'' processing (joins, grouping, etc.) As such, it's important to correctly calibrate this.} 

A unique advantage of FlorDB's replay mechanism lies in its ability to leverage time measurements from the initial run to accurately estimate the time requirements of subsequent replays. This feature sidesteps the longstanding challenge of cost estimation in the realm of databases. \jmh{Be careful in your claim. Our challenge is akin to calibrating an access method like Sequential Scan or Index Scan, which is also pretty easy in traditional cost estimation. The point is not that we solve hard problems in selectivity estimation, but rather that our challenge is not subject to those hard problems because we're at the leaves of the plan tree. Having said that, how do we know how much work we need to do for an index lookup or range scan?}

This estimation process may require calibration when the training replay occurs on a different machine or GPU than the original. This scenario necessitates a calibration step that measures the new machine's IO read/write specifications, enabling FlorDB to adjust time estimates accordingly. While the accuracy of these estimates might vary when switching between systems due to differences in system characteristics, Flor's calibrated approach provides reasonably close estimates, thereby ensuring a level of predictability in system behavior.

\jmh{Signpost a Future Work item on teaching a query optimizer how to use these costs. The discussion in Future Work should be one of simple engineering: if we integrate FlorDB's cost estimates into a traditional cost-based optimizer (e.g. postgres), the optimizer will naturally apply traditional optimizations that minimize data access: selection pushdown to encourage the use of indexes where beneficial, the use of index joins, etc. All that is in the optimizer's search space already, it just needs the cost estimates from us, and ours are even more accurate than usual. So it's not a research problem, it's a matter of engineering.}

==> sections/version_control.tex <==
\subsection{Version Control Architecture}
% Justification and rationale happens in an earlier section.

% TODO: Pseudo-code for autosave.

FLOR autosaves the working directory of the model training project after each run.
Autosave is implemented as a commit into a shadow branch of the current branch in the same repository.
This design protects the current branch from automatic commits with unintelligible commit messages,
and at the same time saves every version of code that executed throughout the existence of the project.
The shadow branch tracks its owner branch,
and the commit hash of the commit from where each execution originated.

% Follow-set. 
% The shadow commit happens at the end of the execution, not at the beginning.

\smallitem{Record-Replay} with shadow branches. To record, the model developer runs the script passing in a flor flag.
To replay, the model developer switches to a shadow branch,
selects a commit, and re-runs the code.
In this sense, the commit is \textit{like} a sandboxed environment.
Shadow-based replay reduces some of the technical debt associated with hindsight logging.
The model developer may modify the script in-place without a destrcutive operation.
Additional files generated neither overwrite or pollute the workspace, and so on.
Autosave by default. Commit message, tag, and branch is post-hoc markup.

\smallitem{Autosave} Flor will save the working directory on every execution.
The reproducibility case.

\smallitem{Shadow branches} The flor CLI flag should map commands to git.
Every shadow branch belongs to one and only one main branch.
Suppose that two main branches merge,
what does this mean for the shadow branch,
forced merge?
What if there is one global "shadow branch" and it is
a stream of executions,
problem is that there may be very sudden changes between versions.
You autosave to a shadow branch.

\smallitem{Ownership and Idenity} Every shadow branch is owned by one and only one primary branch.
When two primary branches merge ...
When a primary branch branches into two, the new branch inherits the autosaves of the previous? By soft linking... sure.

\subsubsection{Beyond GIT}
% Domain-specific shorthands for power-user git
% Make 2 branches...
Now that we have described the version control architecture,
we discuss additional functionality beyond what is provided with Git.
Specifically, we cover the case when the model developer does all of their initial development
in a single branch (e.g. ``main''), and, post-hoc, adds commit messages,
branches, and tags to the repository. Think of this as
exploring a single sequence of alternatives on the main branch,
without thinking specifically of version control.
The tool automatically manages version control in a shadow branch,
even if the model developer didn't even commit once.

Trully distributed version control.
Unlike traditional software, where there is an expectation
that there will be one primary branch,
that will improve with quality over time, in machine learning,
there is no such expectation.
It is at the same time necessary to keep track of multiple alternatives,
and for one patch to make it to all. Keep all architectures current.
To do this, we build (export) a branch (as a single commit)
into our current repository.

In this scenario,
you do a bunch (sequence) of runs
you forget all about git.
Post-hoc, you have the ``main'' branch without any commits (because you forgot).
But because of flor, there is also a ``shadow::main'' with dozens of commits
corresponding to your past runs.
You want to compete two branches to see which is better at your problem.
Your other branch (somewhere in the middle) against the HEAD of the repo.
You checkout the other branch as a commit into a true branch.
And then you apply the fast-forward updates so that they both do the
best and latest data prep.
You name the new branch so-and-so.


